Grassmannian Optimization for Online Tensor Completion and Tracking with the t-SVD

We propose a new fast streaming algorithm for the tensor completion problem of imputing missing entries of a low-tubal-rank tensor using the tensor singular value decomposition (t-SVD) algebraic framework. We show the t-SVD is a specialization of the well-studied block-term decomposition for third-order tensors, and we present an algorithm under this model that can track changing free submodules from incomplete streaming 2-D data. The proposed algorithm uses principles from incremental gradient descent on the Grassmann manifold of subspaces to solve the tensor completion problem with linear complexity and constant memory in the number of time samples. We provide a local expected linear convergence result for our algorithm. Our empirical results are competitive in accuracy but much faster in compute time than state-of-the-art tensor completion algorithms on real applications to recover temporal chemo-sensing and MRI data under limited sampling.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{subcaption}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

\usepackage{bm}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% \usepackage[hidelinks]{hyperref}
% \usepackage[capitalise]{cleveref}
\crefname{equation}{}{}
\Crefname{equation}{Equation}{Equations}
\crefname{figure}{Fig.}{Figs.}

\newtheorem{defn}[theorem]{Definition}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}
\newcommand{\davoud}[1]{{\color{cyan}{[DA: #1]}}}

% Sets running headers as well as PDF title and authors
\headers{Online Tensor Completion with the t-SVD and BTD}{K. Gilman, L. Balzano}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Grassmannian Optimization for Online Tensor Completion and Tracking in the t-SVD and $(L,L,1)$-Block-Term Decomposition Algebras}
%\thanks{Submitted to the editors DATE.
%\funding{This work was funded by _________. }}

% Authors: full names plus addresses.
\author{Kyle Gilman\thanks{University of Michigan, Ann Arbor, MI 
  (\email{kgilman@umich.edu}).}
\and Laura Balzano\thanks{University of Michigan, Ann Arbor, MI 
  (\email{girasole@umich.edu}).}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%% Added on Overleaf: enabling xr
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}% latexmk will find this if $recorder=0 (however, in that case, it will ignore #1 if it is a .aux or .pdf file etc and it exists! if it doesn't exist, it will appear in the list of dependents regardless)
  \@addtofilelist{#1}% if you want it to appear in \listfiles, not really necessary and latexmk doesn't use this
  \IfFileExists{#1}{}{\typeout{No file #1.}}% latexmk will find this message if #1 doesn't exist (yet)
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}

\usepackage[normalem]{ulem}
%%% END HELPER CODE
%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> s,alg,arb_missing.tex <==
\subsection{Deriving the objective function}
\label{subsec:derive_obj_fxn}
\new{We begin by writing the problem we wish to solve as a tubal-rank-$r$ problem in t-SVD notation, and then we will express it as a $(r,r,1)$-tubal BTD}. In the scenario where the underlying free submodule does not change over time, a natural global optimization problem with squared $\ell_2$ error loss is given as 
\begin{equation}
\begin{aligned}
    \label{eq:toucan_objective_incremental}
    \tensor{\hat{U}},\tensor{\hat{W}} = \argmin_{\substack{\tensor{U} \in \mathbb{R}^{d_1 \times r \times d_3}\\ \tensor{W} \in \mathbb{R}^{r \times T \times d_3}}} \frac{1}{2T} \sum_{t=1}^T \left\|\mathcal{A}_{\Omega_t}(\slice{X}_t - \tensor{U} \tP \slice{W}_t) \right\|^2_F \\
    \text{s.t. } \tensor{U}^T \tP \tensor{U} = \tensor{I}_{rrd_3}
\end{aligned}
\end{equation}
\noindent where $\mathcal{A}_{\Omega_t}(\cdot)$ is the linear operator that extracts the observed samples in the set $\Omega_t$ from each lateral slice in $\tensor{X} = [\slice{X}_1 , \hdots, \slice{X}_{d_2}]$,
% \noindent where $\tensor{X} = [\slice{X}_1 , \hdots, \slice{X}_{d_2}]$ is observed on the set of indices \sloppy $\Omega \subset \{1,\hdots,d_1\} \times \{1,\hdots,d_2\} \times \{1,\hdots,d_3\}$
and $\tensor{I}_{rrd_3}$ is the $r \times r \times d_3$ tensor identity (see Appendix). Since we have concatenated the time slices on the second dimension, let $d_2 = T$.
% Due to the linearity of the t-product in each slice of $\slice{W}_t$ and the separability under the Frobenius norm, we can then rewrite this cost function in terms of each lateral slice $\slice{X}_{t}$ at a time for $t=1,2,\hdots, T$.
% \begin{align}
%     \label{eq:toucan_objective_incremental}
%     \tensor{\hat{U}},\tensor{\hat{W}} = \argmin_{\substack{\tensor{U} \in \mathbb{R}^{d_1 \times r \times d_3}\\ \tensor{W} \in \mathbb{R}^{r \times T \times d_3}}} \frac{1}{2T} \sum_{t=1}^T \|\mathcal{A}_{\Omega_t}(\slice{X}_t - \tensor{U} \tP \slice{W}_t) \|^2_F \\
%     \text{s.t. } \tensor{U}^T \tP \tensor{U} = \tensor{I}_{rrd_3} \nonumber
% \end{align}
% \noindent where $\mathcal{A}_{\Omega_t}(\cdot)$ is the linear operator that extracts the observed samples in the set $\Omega_t$. From \cref{eq:toucan_objective_incremental},
We see it is possible to solve this problem incrementally, as described in \cite{bertsekas}, in terms of the orthonormal free-submodule $\tensor{U}$ and the weights $\slice{W}_t \in \mathbb{R}^{r \times 1 \times d_3}$ for all  $t=1,\hdots,T$.

% The problem in (\ref{eq:toucan_objective_incremental}) is an optimization problem on the \textit{tensor Grassmann manifold}, which we define below. \cite{josh_girson} gave that the set of three-ways tensors form a smooth embedded manifold $\mathcal{M}$ of $\mathbb{R}^n$ that can be realized as a real product manifold of rank-$r$ matrices in the Fourier domain.

% \begin{lemma}[Cartesian product of manifolds]\cite{absil_mahony_sepulchre,josh_girson}
%     Let $\mathcal{M}_r^i$ be the $i^{\text{th}}$ smooth manifold of dimension $r$. Then the Cartesian product of $n$ smooth manifolds $\mathcal{M}$ is itself a smooth manifold.
%     \begin{equation}
%         \mathcal{M} = \mathcal{M}_r^1 \times \hdots \times \mathcal{M}_r^n
%     \end{equation}
%     \label{lemma:cartesian_product}
% \end{lemma}
% \vspace{-5mm}

% \begin{theorem}[Tensor Grassmann Manifold]
%     Let $\tensor{U} \in \mathbb{R}^{d_1 \times r \times d_3}$ be an orthonormal tensor and $\tUb \in \mathbb{C}^{d_1 \times r \times d_3}$ be the result of taking the Fourier transform of each tube in $\tensor{U}$. Let $\mathcal{G}_r^{(i)}$ be a Grassmann manifold of dimension $r$ over $\mathbb{C}^{d_1}$ for the frontal face at index $i$. Then from Lemma \ref{lemma:cartesian_product}, $\tUb$ lies on the tensor Grassmann manifold $\mathcal{G}$ that is the set of all free submodules of dimension $r$ in $\mathbb{M}^{d_1}_{d_3}$:
%     \vspace{-3mm}
    
%     \begin{equation}
%         \tUb \in \mathcal{G} = \mathcal{G}_r^{(1)} \times \hdots \times \mathcal{G}_r^{(d_3)}
%     \end{equation}

% \end{theorem}

% We note here that $\tensor{U}$ is one choice of representation for a point on the tensor Grassmannian where the Fourier transform along its tubes $\tUb$ has as each frontal face a matrix with orthonormal columns. However, we can equivalently represent this point using an $d_1 d_3 \times r d_3$ block-diagonal matrix in the Fourier domain, with the frontal faces of $\tUb$ on the diagonal. We will revisit this representation below.

We minimize the cost function in \cref{eq:toucan_objective_incremental} for each slice $\slice{X}_t$ in an alternating fashion with stochastic gradient descent. Let $\cL_t(\tensor{U},\slice{W}_t) = \frac{1}{2} \|\mathcal{A}_{\Omega_t}(\slice{X}_t - \tensor{U} \tP \slice{W}_t) \|^2_F$. Then the objective in \cref{eq:toucan_objective_incremental} is $\frac{1}{2T} \sum_{t=1}^T \cL_t(\tensor{U},\slice{W}_t)$. We will take a stochastic gradient step for each $\cL_t$ sequentially. From the result in \cref{thm:tsvd_btd_equivalency}, we express the objective in each slice at time $t$ as a \new{$(r,r,1)$-tubal BTD in terms of orthonormal bases $\Ub_k \in \C^{d_1 \times r}$ (the frontal faces of $\tU \times_3 \FF_{d_3}$) and the column vectors $\wb_{t,k} \in \C^{r}$  (the frontal faces of $\slice{W}_t \times_3 \FF_{d_3}$):}
% \vspace{-5mm}
\begin{equation}
\begin{aligned}
   \label{eq:arb_missing:btd_stochastic_objective}
   &\cL_t(\tensor{U},\slice{W}_t) = \left\|\PP_{\Omega_t} \texttt{vec}\left(\slice{X}_t - \sum_{k=1}^{d_3} (\Ub_k \wb_{t,k}) \circ \fb_r \right)\right\|_2^2 \\ 
   &= \left\|\FOmeg\left(\begin{bmatrix} \xb_{\Omega_t,1} \\ \vdots \\ \xb_{\Omega_t,d_3} \end{bmatrix} - \begin{bmatrix} \Ub_1 & & 0 \\ & \ddots & \\ 0 & & \Ub_{d_3} \end{bmatrix} \begin{bmatrix} \wb_{t,1} \\ \vdots \\ \wb_{t,d_3} \end{bmatrix}\right)\right\|_2^2.
\end{aligned}
\end{equation}
Above, each $\xb_{\Omega_t,k} \in \C^{d_1}$ denotes the $k^{th}$ frontal face of $\tXb_{\Omega_t} = \new{\Delta_{\Omega_t}(\slice{X}_t)} \times_3 \FF_{d_3}$, where $\Delta_{\Omega_t}(\cdot)$ imputes zeros on the missing coordinates. $\PP_{\Omega_t}$ is a subsampled identity matrix of size $|\Omega_t| \times d_1d_3$, and $\FOmeg := \PP_{\Omega_t} (\FF_{d_3}' \otimes \I_{d_1}) \in \C^{|\Omega_t| \times d_1d_3}$, which in the t-SVD framework is the subsampled inverse Fourier transform. The proof of \cref{eq:arb_missing:btd_stochastic_objective} is left to \cref{appendix:sec:derive_objective_fxn}, along with the proof of the relation using t-SVD algebra in \cref{appendix:sec:tsvd_toucan}. We optimize for each block $\Ub_k \in \C^{d_1 \times r}$ and $\wb_{t,k} \in \C^{r}$ at time $t$ in terms of the vectorized tensor slice $\tXb_{\Omega_t}$. 
% \begin{equation}
% \label{eq:arb_missing:stoch_obj:unitary_C}
%     \cL_t(\tensor{U},\slice{W}_t) = \left\|\PP_{\Omega_t}(\CC \otimes \I_{d_1})\left(\begin{bmatrix} \Xb_1 \\ \vdots \\ \Xb_{d_3} \end{bmatrix} - \begin{bmatrix} \Ub_1 & & 0 \\ & \ddots & \\ 0 & & \Ub_{d_3} \end{bmatrix} \begin{bmatrix} \Wb'_{1_t} \\ \vdots \\ \Wb'_{{d_3}_t} \end{bmatrix}\right)\right\|_2^2.
% \end{equation}

Let us denote $\xb_t := \texttt{vec}(\tXb_{\Omega_t}) \in \C^{d_1d_3}$, $\wb_t := \texttt{vec}(\slice{W}_t \times_3 \FF_{d_3}) \in \C^{d_3r}$, and recall that $\Ub$ denotes the block-diagonal matrix. The objective rewritten is simply
\begin{align}
    \label{eq:toucan_new_obj}
    \cL_t(\tensor{U},\slice{W}_t) = \frac{1}{2} \|\FOmeg (\xb_t - \Ub \wb_t)\|^2_2.
\end{align}
% where $\Ub$ is the block-diagonal matrix with the $d_3$ frontal slices of $\tUb = \tensor{U} \times_3 \FF_{d_3}$ on the diagonal, whose sizes are $d_1 \times k$. This representation requires an additional constraint, that the elements not on these diagonal blocks must be zero. We define the convex set $\mathcal{K}$ to represent these matrices (without any orthogonality constraint).

% \new{\noindent where $\Ub$ is the block-diagonal matrix with the $d_3$ frontal slices of $\tUb = \tensor{U} \times_3 \FF_{d_3}$ on the diagonal, whose sizes are $d_1 \times k$. Observe that due to the coupling between the orthonormal matrices $\Ub_r$ and the weights $\Wb_{t,r}'$ in Euclidean space, $\Ub$ is only determined up to an action of $\mathcal{O}(k) \times \hdots \times \mathcal{O}(k)$ applied to the block diagonals, i.e. each $\Ub_r$ is only determined up to an orthogonal rotation of its columns by $\mathcal{O}(k)$. Thus, define $\Ub_r \in \mathcal{G}(k,d_1) \quad \forall r=1,\hdots,d_3$, where $\mathcal{G}(k,d_1)$ denotes the Grassmannian-- the set of all subspaces of dimension $k$ embedded in $\F^{d_1}$. Subsequently, we reduce \cref{eq:toucan_new_obj} to a minimization problem over a product of $d_3$ Grassmannians $\mathcal{G}_1(k,d_1) \times \hdots \times \mathcal{G}_{d_3}(k,d_1)$, represented by $\Ub$, and a Euclidean space in $\wb$.}

% This is a nonconvex function because of both the biconvexity between $\Ub$ and $\wb$ and the orthonormality constraint $\Ub'\Ub = \I_r$. Our stochastic gradient procedure will fix $\Ub$ and then minimize $\cL_t(\tensor{U},\slice{W}_t)$ with respect to $\wb$ (equivalently $ \Wb_t$); then we fix $\wb$ and take a step in the negative gradient direction of $\cL_t(\tensor{U},\slice{W}_t)$ with respect to $\Ub$ (equiv. $\tensor{U}$). Note that $\Ub_r \in \mathcal{G}(k,d_1) \quad \forall r=1,\hdots,d_3$, where $\mathcal{G}(k,d_1)$ denotes the Grassmannian-- the set of all subspaces of dimension $k$ embedded in $\F^{d_1}$.
% In the t-SVD, updating the free-submodule $\Ub$ involves a projected gradient descent step onto the set of block-diagonal matrices in the Fourier domain followed by a geodesic step along each complex Grassmann manifold in the product of manifolds.

This is a nonconvex function because of both the biconvexity between each $\Ub_k$ and $\wb_{t,k}$ and the orthonormality constraints $\{\Ub_k'\Ub_k = \I_r\}_{k=1}^{d_3}$. \new{Denote $\mathcal{G}(r,d_1)$ as the complex Grassmannian -- the set of all subspaces of dimension $r$ embedded in $\C^{d_1}$ -- and $\mathcal{O}(r)$ as the $r$-dimensional orthogonal group:
\begin{align}
    \mathcal{G}(r,d) &= \{\U \RR: \U \in \C^{d \times r}, \U'\U = \I_r, \RR \in \mathcal{O}(r)\}, \\
    \mathcal{O}(r) &= \{\RR \in \C^{r \times r}, \RR'\RR = \RR \RR' = \I_r \}.
\end{align}
}

% \new{Recall that $\Ub$ is the block-diagonal matrix with the $d_3$ frontal slices of $\tUb = \tensor{U} \times_3 \FF_{d_3}$ on the diagonal, whose sizes are $d_1 \times r$. Observe that due to the coupling between the orthonormal matrices $\Ub_k$ and the weights $\Wb_{k}'$ in Euclidean space, $\Ub$ is only determined up to an action of $\mathcal{O}(r) \times \hdots \times \mathcal{O}(r)$ applied to the block diagonals, i.e. each $\Ub_k$ is only determined up to an orthogonal rotation of its columns by $\mathcal{O}(r)$. Thus, define $\Ub_k \in \mathcal{G}(r,d_1) \quad \forall k=1,\hdots,d_3$, and we will minimize a problem over a product of $d_3$ Grassmannians $\mathcal{G}_1(r,d_1) \times \hdots \times \mathcal{G}_{d_3}(r,d_1)$ (represented by $\Ub$) and a Euclidean space in the weights.}

\new{Observe that due to the coupling between the orthonormal matrices $\Ub_k$ and the weights $\wb_{k}$ in Euclidean space, each $\Ub_k$ is only determined up to an orthogonal rotation of its columns by $\mathcal{O}(r)$. Thus, define $\Ub_k \in \mathcal{G}(r,d_1) \quad \forall k=1,\hdots,d_3$, and we will minimize a problem over a product of $d_3$ Grassmannians $\mathcal{G}_1(r,d_1) \times \hdots \times \mathcal{G}_{d_3}(r,d_1)$ (represented by $\Ub$, which is the block-diagonal matrix with the $d_3$ frontal slices of $\tUb = \tensor{U} \times_3 \FF_{d_3}$ on the diagonal, whose sizes are $d_1 \times r$) and a Euclidean space in the weights.}



Our stochastic gradient procedure will fix $\Ub$ and then minimize $\cL_t(\tensor{U},\slice{W}_t)$ with respect to $\wb_t$ (equivalently $\slice{W}_t$); then we fix $\wb_t$ and take a step in the negative gradient direction of $\cL_t(\tensor{U},\slice{W}_t)$ \new{ with respect to each block $\Ub_k$ on the diagonal of $\Ub$ (equiv. $\tensor{U}$). 
In the t-SVD, updating the free-submodule $\Ub$ involves stochastic gradient descent by a geodesic step along each complex Grassmann manifold $\mathcal{G}_k(r,d_1)$ in the product of manifolds.}









==> s,alg,arb_missing_v2.tex <==
\subsection{Deriving the objective function}
\label{subsec:derive_obj_fxn}

\textcolor{red}{Old version}

\new{We begin by writing the problem we wish to solve as a tubal-rank-$r$ problem in t-SVD notation, and then we will express it as a $(r,r,1)$-tubal BTD}. In the scenario where the underlying free submodule does not change over time, a natural global optimization problem with squared $\ell_2$ error loss is given as 
% \begin{equation}
% \begin{aligned}
%     \label{eq:toucan_objective_incremental}
%     \tensor{\hat{U}},\tensor{\hat{W}} = \argmin_{\substack{\newnew{[\tensor{U}] \in \mathcal{G}(r,d_1,d_3)} \\ \tensor{W} \in \mathbb{R}^{r \times T \times d_3}}} \frac{1}{2T} \sum_{t=1}^T \left\|\mathcal{A}_{\Omega_t}(\slice{X}_t - \tensor{U} \tP \slice{W}_t) \right\|^2_F
% \end{aligned}
% \end{equation}
% {
% \color{blue}
% \begin{equation}
% \begin{aligned}
%     \label{eq:toucan_objective_incremental}
%     \tensor{\hat{U}},\tensor{\hat{W}} = &\argmin_{\substack{\newnew{[\tensor{U}] \in {\mathcal{G}(r,d_1,d_3)}} \\ \tensor{W} \in \mathbb{R}^{r \times T \times d_3}}} \cL(\tU,\tW)\\
%     &\cL(\tU,\tW) := \frac{1}{2T} \sum_{t=1}^T \left\|\mathcal{A}_{\Omega_t}(\slice{X}_t - \tensor{U} \tP \slice{W}_t) \right\|^2_F.
% \end{aligned}
% \end{equation}
% }
{
\color{blue}
\begin{equation}
\begin{aligned}
\begin{split}
    \label{eq:toucan_objective_incremental}
    &\min_{[\tensor{U}] \in {\mathcal{G}(r,d_1,d_3)}} \clL(\tU), \qquad \clL(\tU) := \frac{1}{T} \sum_{t=1}^T \cL_t(\tU)\\
    &\cL_t(\tU) := \min_{\slice{W}_t \in \R^{r \times 1 \times d_3}} \frac{1}{2}\left\|\mathcal{A}_{\Omega_t}(\slice{X}_t - \tensor{U} \tP \slice{W}_t) \right\|^2_F.
\end{split}
\end{aligned}
\end{equation}
}
where $\mathcal{A}_{\Omega_t}(\cdot)$ is the linear operator that extracts the observed samples in the set $\Omega_t$ from each lateral slice in $\tensor{X} = [\slice{X}_1 , \hdots, \slice{X}_{d_2}]$, \newnew{and $\mathcal{G}(r,d_1,d_3)$ denotes the t-Grassmannian -- a smooth compact manifold; see, \cref{def:tensor_grassmannian} and \cref{propzer:well_defined_tensor_grassmannian}. 

% The following proposition shows that i) $\slice{W}_t$ is  the unique minimizer to $\overline{\cL}_t(\tUb)$ as long as  $((\FOmeg \Ub)'(\FOmeg \Ub))^{-1}$ remains full rank; and ii) $\cL :\mathcal{G}(r,d_1,d_3) \times \mathbb{R}^{r \times T \times d_3} \rightarrow \mathbb{R}$ is a well-defined smooth function.


% Let $\wb_t = \argmin_{\ab \in \mathbb{C}^{d_3r}} \frac{1}{2} \|\FOmeg (\xb_t - \Ub\ab)\|^2_2.$ So long as we sample enough entries of the data such that $((\FOmeg \Ub)'(\FOmeg \Ub))^{-1}$ remains full rank, then $\wb_t$ is the unique minimizer to $\overline{\cL}_t(\tUb)$.




}

% The problem in (\ref{eq:toucan_objective_incremental}) is an optimization problem on the \textit{tensor Grassmann manifold}, which we define below. \cite{josh_girson} gave that the set of three-ways tensors form a smooth embedded manifold $\mathcal{M}$ of $\mathbb{R}^n$ that can be realized as a real product manifold of rank-$r$ matrices in the Fourier domain.

% \begin{lemma}[Cartesian product of manifolds]\cite{absil_mahony_sepulchre,josh_girson}
%     Let $\mathcal{M}_r^i$ be the $i^{\text{th}}$ smooth manifold of dimension $r$. Then the Cartesian product of $n$ smooth manifolds $\mathcal{M}$ is itself a smooth manifold.
%     \begin{equation}
%         \mathcal{M} = \mathcal{M}_r^1 \times \hdots \times \mathcal{M}_r^n
%     \end{equation}
%     \label{lemma:cartesian_product}
% \end{lemma}
% \vspace{-5mm}

% \begin{theorem}[Tensor Grassmann Manifold]
%     Let $\tensor{U} \in \mathbb{R}^{d_1 \times r \times d_3}$ be an orthonormal tensor and $\tUb \in \mathbb{C}^{d_1 \times r \times d_3}$ be the result of taking the Fourier transform of each tube in $\tensor{U}$. Let $\mathcal{G}_r^{(i)}$ be a Grassmann manifold of dimension $r$ over $\mathbb{C}^{d_1}$ for the frontal face at index $i$. Then from Lemma \ref{lemma:cartesian_product}, $\tUb$ lies on the tensor Grassmann manifold $\mathcal{G}$ that is the set of all free submodules of dimension $r$ in $\mathbb{M}^{d_1}_{d_3}$:
%     \vspace{-3mm}
    
%     \begin{equation}
%         \tUb \in \mathcal{G} = \mathcal{G}_r^{(1)} \times \hdots \times \mathcal{G}_r^{(d_3)}
%     \end{equation}

% \end{theorem}

% We note here that $\tensor{U}$ is one choice of representation for a point on the tensor Grassmannian where the Fourier transform along its tubes $\tUb$ has as each frontal face a matrix with orthonormal columns. However, we can equivalently represent this point using an $d_1 d_3 \times r d_3$ block-diagonal matrix in the Fourier domain, with the frontal faces of $\tUb$ on the diagonal. We will revisit this representation below.

Since we have concatenated the time slices on the second dimension, let $d_2 = T$. We see it is possible to solve this problem incrementally, as described in \cite{bertsekas}, in terms of the orthonormal free-submodule $\tensor{U}$ and the \newnew{optimal} weights $\slice{W}_t \in \mathbb{R}^{r \times 1 \times d_3}$ for all  $t=1,\hdots,T$. We minimize the cost function in \cref{eq:toucan_objective_incremental} for each slice $\slice{X}_t$ with stochastic gradient descent. From the results in \cref{thm:tsvd_btd_equivalency} \newnew{and \cref{prop:well_defined_tensor_grassmannian}}, we express each $\clL_t(\tU)$ in each slice at time $t$ as a \new{$(r,r,1)$-tubal BTD in terms of \newnew{$[\Ub_k] \in \overline{\mathcal{G}}(r,d_1)$}  and the column vectors $\wb_{t,k} \in \C^{r}$ for $k=1,\hdots,d_3$, i.e. the frontal faces of $\tUb = \tU \times_3 \FF_{d_3}$ and $\tWb_t = \slice{W}_t \times_3 \FF_{d_3}$, respectively. Let $\overline{\clL}_t$ denote each $\cL_t$ expressed in its Fourier variables, recalling that $\Ub$ denotes the block-diagonal matrix representation of $\tUb$:}
% \vspace{-5mm}

\begin{align}
% \begin{split}
   \label{eq:arb_missing:btd_stochastic_objective}
% &\newnew{\min_{\substack{[\Ub_k] \in \overline{\mathcal{G}}(r,d_1),~\forall k\in[d_3]~\hspace{1mm} \\ 
%           \tensor{\widebar{W}} \in \mathbb{C}^{r \times T \times d_3}}} \frac{1}{2T} \sum_{t=1}^T \overline{\cL}_t(\tUb,\tWb_t)} \\
    & \newthree{\min_{[\Ub_k] \in \overline{\mathcal{G}}(r,d_1),~\forall k\in[d_3]}} \frac{1}{T} \sum_{t=1}^T \overline{\cL}_t(\Ub) \\
   &\overline{\cL}_t(\Ub) = \newthree{\min_{\wb_t}} \frac{1}{2}\left\|\PP_{\Omega_t} \texttt{vec}\left(\slice{X}_t - \sum_{k=1}^{d_3} (\Ub_k \wb_{t,k}) \circ \fb_r \right)\right\|_2^2 \notag \\ 
   &= \newthree{\min_{\wb_t}} \frac{1}{2} \left\|\FOmeg\left(\begin{bmatrix} \xb_{\Omega_t,1} \\ \vdots \\ \xb_{\Omega_t,d_3} \end{bmatrix} - \begin{bmatrix} \Ub_1 & & 0 \\ & \ddots & \\ 0 & & \Ub_{d_3} \end{bmatrix} \begin{bmatrix} \wb_{t,1} \\ \vdots \\ \wb_{t,d_3} \end{bmatrix}\right)\right\|_2^2. \notag 
%   \end{split}
\end{align}

Above, each $\xb_{\Omega_t,k} \in \C^{d_1}$ denotes the $k^{th}$ frontal face of $\tXb_{\Omega_t} = \new{\Delta_{\Omega_t}(\slice{X}_t)} \times_3 \FF_{d_3}$, where $\Delta_{\Omega_t}(\cdot)$ imputes zeros on the missing coordinates. $\PP_{\Omega_t}$ is a subsampled identity matrix of size $|\Omega_t| \times d_1d_3$, and $\FOmeg := \PP_{\Omega_t} (\FF_{d_3}' \otimes \I_{d_1}) \in \C^{|\Omega_t| \times d_1d_3}$, which in the t-SVD framework is the subsampled inverse Fourier transform. The proof of \cref{eq:arb_missing:btd_stochastic_objective} is left to \cref{appendix:sec:derive_objective_fxn}, along with the proof of the relation using t-SVD algebra in \cref{appendix:sec:tsvd_toucan}. 

% We optimize for each block $\Ub_k \in \C^{d_1 \times r}$ and $\wb_{t,k} \in \C^{r}$ at time $t$ in terms of the vectorized tensor slice $\tXb_{\Omega_t}$. 
% \begin{equation}
% \label{eq:arb_missing:stoch_obj:unitary_C}
%     \cL_t(\tensor{U},\slice{W}_t) = \left\|\PP_{\Omega_t}(\CC \otimes \I_{d_1})\left(\begin{bmatrix} \Xb_1 \\ \vdots \\ \Xb_{d_3} \end{bmatrix} - \begin{bmatrix} \Ub_1 & & 0 \\ & \ddots & \\ 0 & & \Ub_{d_3} \end{bmatrix} \begin{bmatrix} \Wb'_{1_t} \\ \vdots \\ \Wb'_{{d_3}_t} \end{bmatrix}\right)\right\|_2^2.
% \end{equation}

Let us denote $\xb_t := \texttt{vec}(\tXb_{\Omega_t}) \in \C^{d_1d_3}$, $\wb_t := \texttt{vec}(\slice{W}_t \times_3 \FF_{d_3}) \in \C^{d_3r}$. Then
\begin{align}
    \label{eq:toucan_new_obj}
    \overline{\cL}_t(\Ub) = \textcolor{blue}{\min_{\wb_t}} \frac{1}{2} \|\FOmeg (\xb_t - \Ub \wb_t)\|^2_2.
\end{align}
% where $\Ub$ is the block-diagonal matrix with the $d_3$ frontal slices of $\tUb = \tensor{U} \times_3 \FF_{d_3}$ on the diagonal, whose sizes are $d_1 \times k$. This representation requires an additional constraint, that the elements not on these diagonal blocks must be zero. We define the convex set $\mathcal{K}$ to represent these matrices (without any orthogonality constraint).

% \new{\noindent where $\Ub$ is the block-diagonal matrix with the $d_3$ frontal slices of $\tUb = \tensor{U} \times_3 \FF_{d_3}$ on the diagonal, whose sizes are $d_1 \times k$. Observe that due to the coupling between the orthonormal matrices $\Ub_r$ and the weights $\Wb_{t,r}'$ in Euclidean space, $\Ub$ is only determined up to an action of $\mathcal{O}(k) \times \hdots \times \mathcal{O}(k)$ applied to the block diagonals, i.e. each $\Ub_r$ is only determined up to an orthogonal rotation of its columns by $\mathcal{O}(k)$. Thus, define $\Ub_r \in \mathcal{G}(k,d_1) \quad \forall r=1,\hdots,d_3$, where $\mathcal{G}(k,d_1)$ denotes the Grassmannian-- the set of all subspaces of dimension $k$ embedded in $\F^{d_1}$. Subsequently, we reduce \cref{eq:toucan_new_obj} to a minimization problem over a product of $d_3$ Grassmannians $\mathcal{G}_1(k,d_1) \times \hdots \times \mathcal{G}_{d_3}(k,d_1)$, represented by $\Ub$, and a Euclidean space in $\wb$.}

% This is a nonconvex function because of both the biconvexity between $\Ub$ and $\wb$ and the orthonormality constraint $\Ub'\Ub = \I_r$. Our stochastic gradient procedure will fix $\Ub$ and then minimize $\cL_t(\tensor{U},\slice{W}_t)$ with respect to $\wb$ (equivalently $ \Wb_t$); then we fix $\wb$ and take a step in the negative gradient direction of $\cL_t(\tensor{U},\slice{W}_t)$ with respect to $\Ub$ (equiv. $\tensor{U}$). Note that $\Ub_r \in \mathcal{G}(k,d_1) \quad \forall r=1,\hdots,d_3$, where $\mathcal{G}(k,d_1)$ denotes the Grassmannian-- the set of all subspaces of dimension $k$ embedded in $\F^{d_1}$.
% In the t-SVD, updating the free-submodule $\Ub$ involves a projected gradient descent step onto the set of block-diagonal matrices in the Fourier domain followed by a geodesic step along each complex Grassmann manifold in the product of manifolds.


\textcolor{blue}{
\begin{proposition}
\label{prop:well_defined_tensor_grassmannian}
Suppose $|\Omega_t|$ is sufficiently large  such that $((\FOmeg \Ub)'(\FOmeg \Ub))^{-1}$ remains full rank. Then,
\begin{itemize}
    \item the inner least-squares problem with respect to $\slice{W}_t$ has a unique solution.  %$\slice{W}_t$ is  the unique minimizer to ${\cL}_t(\tU)$,
%     \item $\mathcal{G}(r,d_1,d_3) $ is a smooth compact manifold of {
% \color{blue} dimension $d_3r(d_1-r)$}.  
\item  $\clL$ is a well-defined smooth function over  $\mathcal{G}(r,d_1,d_3)$ and it admits a global optimizer. 
\end{itemize}
\end{proposition}
We leave the proof of \cref{prop:well_defined_tensor_grassmannian} to \cref{appendix:proof:prop:well_defined_tensor_grassmannian}. At a high level, the proof shows that the optimization problem constrained to $[\tU] \in \mathcal{G}(r,d_1,d_3)$ is a well-defined problem on a product manifold of Grassmannians in the Fourier domain.
}

The problem in \cref{eq:arb_missing:btd_stochastic_objective} is nonconvex from the biconvexity between each $\Ub_k$ and $\wb_{t,k}$ and the orthonormality constraints $\Ub_k'\Ub_k = \I_r$ for all $k \in [d_3]$. We will minimize a problem over a product of $d_3$ Grassmannians $\mathcal{G}_1(r,d_1) \times \hdots \times \mathcal{G}_{d_3}(r,d_1)$ (represented by $\Ub$, which is the block-diagonal matrix with the $d_3$ frontal slices of $\tUb = \tensor{U} \times_3 \FF_{d_3}$ on the diagonal, whose sizes are $d_1 \times r$). For a single data observation, we first find the unique minimizer $\wb_t$ (equivalently $\slice{W}_t$) to the inner least-squares problem, and then take a stochastic gradient descent step of the outer problem in the negative gradient direction of $\overline{\cL}_t(\tUb)$ with respect to each block $\Ub_k$ on the diagonal of $\Ub$ for estimating $\tUb$ (equivalently $\tU$).

% Our stochastic gradient procedure will fix $\Ub$ and then minimize $\overline{\cL}_t(\tUb,\tWb_t)$ with respect to $\wb_t$ (equivalently $\slice{W}_t$); then we fix $\wb_t$ and take a step in the negative gradient direction of $\overline{\cL}_t(\tUb,\tWb_t)$ \new{ with respect to each block $\Ub_k$ on the diagonal of $\Ub$ (equiv. $\tensor{U}$). 
% In the t-SVD, updating the free-submodule $\Ub$ involves stochastic gradient descent by a geodesic step along each complex Grassmann manifold $\mathcal{G}_k(r,d_1)$ in the product of manifolds.}











==> s,experiments_cgd_bound.tex <==
We demonstrate that TOUCAN empirically obeys our derived upper bound from Theorem \ref{thm:sample_bound} (or Equation \ref{eq:sample_ub}). We generate a small problem of synthetic data of size $n_1 = 50, n_2 = 200, n_3 = 20$ with tubal-rank 5 from a synthetic FSM $\tensor{U}_0\in\mathbb{R}^{n_1 \times r \times n_3}$. We construct the full matrix $\mathcal{F}_{\Omega_t}\bar{U_0}$ and compute the average $\kappa(\mathcal{F}_{\Omega_t}\bar{U_0})^2$ for 20 random sampling patterns for each sampling rate and use this to compute the CGD sample bound. We also plot our bound derived in Theorem \ref{thm:sample_bound}. We let TOUCAN process the data and record the average number of CGD iterations per algorithm iteration. We plot the results in Fig. \ref{fig:cgd_iter_plot} along with the recovered tensor NRMSE; the horizontal axis is ${dof} / |\Omega|$ where $dof = n_3r((n_1 + n_2) - r)$ is the degrees of freedom of the set of tubal-rank $r$ tensors and $|\Omega|$ again is the number of observed samples. We do not plot the empirical number of CGD iterations above 300. We observe two regions of interest--one where the number of CGD iterations is near-linear as a function of the sampling rate, and one where the number of iterations exponentially increases as the data becomes highly undersampled. It is in this transition we see TOUCAN's completion ability begins to fail. While our bound is fairly tight in the linear region, it is quite loose in the highly-undersampled regime.
 
%  \begin{figure}
%      \centering
%      \includegraphics[width=0.5\textwidth]{figures/synthetic/cgd_iter_vs_sample5-50-20.eps}
%      \caption{Number of average conjugate gradient iterations per TOUCAN iteration with varying sampling rates. We compare to the empirical bound based on the computed condition number and the bound in Theorem \ref{thm:sample_bound}. The right plot shows the recovery error by sampling rate.}
%      \label{fig:cgd_iter_plot}
%  \end{figure}

==> tasks.tex <==
\newcommand{\nextstep}[1]{{\color{blue}#1}}
\section*{Task list \nextstep{(next steps highlighted)}}

\begin{enumerate}

\item Describe related work
\begin{enumerate}
  \item Advantages over other streaming methods?
  \item \sout{Tucker algorithms for completion}
  \item \sout{Streaming tucker algorithms}
  \item \sout{Other missing citations}
\end{enumerate}

\item Experiments
\begin{enumerate}
    \item Finish large scale synthetic experiments
    \item \sout{Make sure logical flow of text is not broken. Sec 5.2.1 methods explained in Section 5.2.2!}
    \item \sout{Check that all algorithm parameters are given.}
    \item \sout{Clean up MRI experiments. Make sure all is there. Try to fit in tables.}
\end{enumerate}

\item Appendix
\begin{enumerate}
    \item \sout{Shorten. Format proofs}
    \item \sout{Fix referencing issues.}
\end{enumerate}

\end{enumerate}

